Optimistic mirror descent in saddle-point problems: Going the extra (gradient) mile

Owing to their connection with generative adversarial networks (GANs), saddle-point problems have recently attracted considerable interest in machine learning and beyond. By necessity, most theoretical guarantees revolve around convex-concave (or even linear) problems; however, making theoretical inroads towards efficient GAN training depends crucially on moving beyond this classic framework. To make piecemeal progress along these lines, we analyze the behavior of mirror descent (MD) in a class of non-monotone problems whose solutions coincide with those of a naturally associated variational inequality - a property which we call coherence. We first show that ordinary, "vanilla" MD converges under a strict version of this condition, but not otherwise; in particular, it may fail to converge even in bilinear models with a unique solution. We then show that this deficiency is mitigated by optimism: by taking an "extra-gradient" step, optimistic mirror descent (OMD) converges in all coherent problems. Our analysis generalizes and extends the results of Daskalakis et al. (2018) for optimistic gradient descent (OGD) in bilinear problems, and makes concrete headway for establishing convergence beyond convex-concave games. We also provide stochastic analogues of these results, and we validate our analysis by numerical experiments in a wide array of GAN models (including Gaussian mixture models, as well as the CelebA and CIFAR-10 datasets).

==> Analysis.tex <==
%----------------------------------------------------------------------
%%% ANALYSIS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


In the analysis of \acl{MD} schemes with convex/monotone objectives, it is customary to consider the so-called \emph{ergodic average}
\begin{equation}
\label{eq:ergodic}
\bar\act_{\run}
	= \frac{\sum_{\runalt=\start}^{\run} \step_{\runalt} \act_{\runalt}}{\sum_{\runalt=\start}^{\run} \step_{\runalt}},
\end{equation}
or some other weighted average of the generated sequence of iterates $\act_{\run}$.
The reason for this is that convexity guarantees \textendash\ via Jensen's inequality and gradient monotonicity \textendash\ that a regret-based analysis of \eqref{eq:SPMD} can yield explicit convergence rates for $\bar\act_{\run}$.
However, this is no longer the case beyond convex-concave problems:
in general, averaging provides no tangible benefits in a non-monotone setting, so we will examine the convergence properties of the ``last iterate'' $\act_{\run}$ of \eqref{eq:SPMD} directly.
\PM{In state-of-the-art (or here), recall that the convergence of \eqref{eq:SPMD} is known for convex-concave objectives (in the sense of ergodic averages) but almost nothing except monotone problems.}

Our starting point is the following energy limit result:

\begin{proposition}
\label{prop:dichotomy}
Suppose that \eqref{eq:SP} is coherent and \eqref{eq:SPMD} is run with a variable step-size $\step_{\run}$ such that $\sum_{\run=\start}^{\infty} \step_{\run}^{2} < \infty$.
If $\sol\in\feas$ is a solution of \eqref{eq:SP}, the Bregman divergence $\breg(\sol,\act_{\run})$ converges \as to a random variable $\breg(\sol)$ with $\exof{\breg(\sol)} < \infty$.
\end{proposition}

\begin{proof}
Let $\breg_{\run} = \breg(\sol,\act_{\run})$ for some solution $\sol$ of \eqref{eq:SP}.
Then, by \cref{prop:Bregman}, we have
\begin{flalign}
\label{eq:Bregman-new-bound}
\breg_{\run+1}
%	= \breg(\sol,\act_{\run+1})
	= \breg(\sol,\prox_{\act_{\run}}(-\step_{\run}\est\gvec_{\run}))
	&\leq \breg(\sol,\act_{\run})
	- \step_{\run} \braket{\est\gvec_{\run}}{\act_{\run} - \sol}
	+ \frac{\step_{\run}^{2}}{2\strong} \norm{\est\gvec_{\run}}^{2}
	\notag\\
	&= \breg_{\run}
	- \step_{\run} \braket{\gvec(\act_{\run})}{\act_{\run} - \sol}
	- \step_{\run} \braket{\noise_{\run}}{\act_{\run} - \sol}
	+ \frac{\step_{\run}^{2}}{2\strong} \dnorm{\est\gvec_{\run}}^{2}
	\notag\\
	&\leq \breg_{\run}
	+ \step_{\run} \snoise_{\run}
	+ \frac{\step_{\run}^{2}}{2\strong} \dnorm{\est\gvec_{\run}}^{2},
\end{flalign}
where, in the last line, we set $\snoise_{\run} = -\braket{\noise_{\run}}{\act_{\run} - \sol}$ and we invoked the assumption that \eqref{eq:SP} is coherent.
Thus, conditioning on $\filter_{\run-1}$ and taking expectations, we get
\PM{Stopped here.}
\begin{flalign}
\exof{\breg_{\run+1} \given \filter_{\run-1}}
	\leq \breg_{\run}
	+ \exof{\snoise_{\run} \given \filter_{\run-1}}
	+ \frac{\step_{\run}^{2}}{2\strong} \exof{\dnorm{\est\gvec_{\run}}^{2} \given \filter_{\run-1}}
%	\notag\\
	\leq \breg_{\run}
	+ \frac{\gbound^{2}}{2\strong} \step_{\run}^{2},
\end{flalign}
where we used \eqref{eq:oracle} and the fact that $\act_{\run}$ is predictable.

Now, letting $R_{\run} = \breg_{\run} + (2\strong)^{-1} \gbound^{2} \sum_{\runalt=\run}^{\infty} \step_{\runalt}^{2}$, the estimate \eqref{eq:Bregman-new-bound} gives
\begin{equation}
\exof{R_{\run+1} \given \filter_{\run}}
	= \exof{\breg_{\run+1} \given \filter_{\run}}
	+ \frac{\gbound^{2}}{2\strong} \sum_{\runalt=\run+1}^{\infty} \step_{\runalt}^{2}
	\leq \breg_{\run}
	+ \frac{\gbound^{2}}{2\strong} \sum_{\runalt=\run}^{\infty} \step_{\runalt}^{2}
	= R_{\run},
\end{equation}
\ie $R_{\run}$ is an $\filter_{\run}$-adapted supermartingale.
Since $\sum_{\run=\start}^{\infty} \step_{\run}^{2} < \infty$, it follows that $\exof{R_{\run}} \leq \exof{R_{\start}} = \exof{\breg_{\start}} + (2\strong)^{-1} \gbound^{2} \sum_{\run=\start}^{\infty} \step_{\run}^{2} < \infty$, \ie $R_{\run}$ is uniformly bounded in $L^{1}$.
Thus, by Doob's convergence theorem for supermartingales \citep[Theorem~2.5]{HH80}, it follows that $R_{\run}$ converges \as to some finite random variable $R_{\infty}$ with $\exof{R_{\infty}} < \infty$.
In turn, by inverting the definition of $R_{\run}$, this shows that $\breg_{\run}$ converges \as to some random variable $\breg(\sol)$ with $\exof{\breg(\sol)} < \infty$, as claimed.
\end{proof}


\cref{prop:dichotomy} can be seen as a ``dichotomy principle'':
it shows that the Bregman divergence is an asymptotic constant of motion, so \eqref{eq:SPMD} either converges to a \acl{SP} $\sol$ (if $\breg(\sol) = 0$) or to some nonzero level set of the Bregman divergence (with respect to $\sol$).
In this way, \cref{prop:dichotomy} rules out more complicated chaotic or aperiodic behaviors that may arise in general.
\PM{G, this could be a good place to discuss/mention our SODA results and your results for chaos.}

However, in making this dichotomy complete, there is a subtlety that arises regarding the level sets of $\breg$.
Specifically, even though $\breg(\base,\act_{\run})$ implies that $\act_{\run}$ converges to $\base$ (by \cref{prop:Bregman}), the converse may fail:
in particular, we could have $\breg(\sol) > 0$ but $\act_{\run}\to\sol$.
For instance, if $\feas$ is the $L^{2}$ ball of $\R^{\vdim}$ and we take $\hreg(\state) = -\sqrt{1 - \norm{\state}_{2}^{2}}$, a straightforward calculation gives
\begin{equation}
\breg(\base,\state)
	= \frac{1 - \braket{\base}{\state}}{\sqrt{1-\norm{\state}_{2}^{2}}}
\end{equation}
whenever $\norm{\base}_{2}=1$.
The corresponding level sets $L_{c}(\base) = \setdef{\state\in\R^{\vdim}}{\breg(\base,\state) = c}$ are then given by the equation
\begin{equation}
1 - \braket{\base}{\state}
	= c \sqrt{1 - \norm{\state}_{2}^{2}},
\end{equation}
which admits $\base$ as a solution for all $c\geq0$ (so $\base$ belongs to the closure of $L_{c}(\base)$ even though $\breg(\base,\base) = 0$ by definition).
As a result, under this choice of regularizer, it is possible to have $\act_{\run}\to\base$ even if $\liminf_{\run\to\infty} \breg(\base,\act_{\run}) > 0$.

To discard such pathologies, we will focus in what follows on distance-generating functions that satisfy the ``reciprocity condition''
\begin{equation}
\label{eq:reciprocity}
\tag{H3}
\breg(\base,\act_{\run})
	\to 0
	\quad
	\text{whenever}
	\quad
	\act_{\run} \to \base,
\end{equation}
for every sequence of points $\act_{\run}\in\dom\subd\hreg$ and all $\base\in\feas$.
This regularity requirement dates back at least to the work of \cite{CT93} who recognized its importance for the convergence analysis of proximal-like methods in convex optimization problems.
For a detailed discussion in the context of convex programming, we refer the reader to \cite{Kiw97b};
we only mention here that our archetypal regularizer examples (\ie \cref{ex:Eucl,ex:entropic}) both satisfy \eqref{eq:reciprocity}.

Now, under \eqref{eq:reciprocity}, the dichotomy principle underlying \cref{prop:dichotomy} becomes complete:
if $\breg(\sol) = 0$, $\act_{\run}$ converges to $\sol$;
otherwise, $\act_{\run}$ converges to an isocline of $\breg$ that lies a positive distance away from $\sol$.
\PM{Can add fluff here about our SODA results, etc.}
However, unless the value of $\breg(\sol)$ can be somehow predicted (or estimated) in advance, this result cannot be easily applied.
To that end, we turn below to a different question, namely whether \eqref{eq:SPMD} gets arbitrarily close to solution of \eqref{eq:SP}:

In view of all this, combining \cref{prop:dichotomy,prop:recurrence} yields the following convergence result:

\begin{theorem}
\label{thm:conv}
Suppose that \eqref{eq:SP} is strictly coherent and \eqref{eq:SPMD} is run with a variable step-size $\step_{\run}$ such that $\sum_{\run=\start}^{\infty} \step_{\run} = \infty$ and $\sum_{\run=\start}^{\infty} \step_{\run}^{2} < \infty$.
Then, under Hypotheses \crefrange{eq:smooth}{eq:reciprocity}, $\act_{\run}$ converges with probability $1$ to a solution of \eqref{eq:SP}.
\end{theorem}

\begin{proof}
By \cref{prop:recurrence}, there exists a solution point $\sol$ of \eqref{eq:SP} such that $\liminf_{\run\to\infty} \breg(\sol,\act_{\run}) = 0$.
Since $\lim_{\run\to\infty} \breg(\sol,\act_{\run})$ exists with probability $1$ (by \cref{prop:dichotomy}), it follows that
\begin{equation}
\lim_{\run\to\infty} \breg(\sol,\act_{\run})
	= \liminf_{\run\to\infty} \breg(\sol,\act_{\run})
	= 0,
\end{equation}
\ie $\act_{\run}$ converges to $\sol$ (by the first part of \cref{prop:Bregman}).
\end{proof}

As an immediate corollary of \cref{thm:conv}, we then obtain:
\begin{corollary}
\label{cor:conv}
Suppose that $\obj$ is strictly convex-concave and \eqref{eq:SPMD} is run with a variable step-size $\step_{\run}$ such that $\sum_{\run=\start}^{\infty} \step_{\run} = \infty$ and $\sum_{\run=\start}^{\infty} \step_{\run}^{2} < \infty$.
Then, under Hypotheses \crefrange{eq:smooth}{eq:reciprocity}, $\act_{\run}$ converges with probability $1$ to the \textpar{necessarily unique} solution of \eqref{eq:SP}.
\end{corollary}

\begin{proof}
By \cref{prop:convex} in \cref{app:aux}, the \acl{SP} problem \eqref{eq:SP} is strictly coherent if $\obj$ is strictly convex-concave.
Our claim thus follows from \cref{thm:conv}.
\end{proof}

On the other hand, if \eqref{eq:SP} is coherent but not \emph{strictly} so, \eqref{eq:SPMD} may fail to converge and instead cycle indefinitely.
\PM{This could be a good point to plug the various instability phenomena observed in \acp{GAN}.}
For concreteness, we present below a very simple class of examples where this phenomenon arises:
finite two-player zero-sum games with an interior equilibrium.

To properly define them, let $\pures_{\play} = \{1,\dotsc,\nPures_{\play}\}$, $\play=1,2$, be two finite sets of \emph{pure strategies}, and let $\feas_{\play} = \simplex(\pures_{\play})$ denote the set of \emph{mixed strategies} of player $\play$.
A \emph{two-player zero-sum game} on $\pures_{1}\times\pures_{2}$ is then defined by a matrix $\mat\in\R^{\pures_{1}\times\pures_{2}}$ such that
\begin{equation}
\label{eq:finite}
\obj(\state_{1},\state_{2})
	= \state_{1}^{\top} \mat \state_{2}
\end{equation}
represents concurrently the loss of Player $1$ and the reward of Player $2$ in the mixed strategy profile $\state = (\state_{1},\state_{2})\in\feas$.
Then, writing $\fingame \equiv \fingame(\pures_{1},\pures_{2},\mat)$ for the resulting game, we have:

\begin{proposition}
\label{prop:finite}
Suppose that $\fingame$ is a two-player zero-sum game with an interior equilibrium $\sol\in\intfeas$.
If \eqref{eq:SPMD} is run with perfect oracle feedback \textpar{$\noisevar=0$} and a step-size $\step_{\run}$ such that $\sum_{\run=\start}^{\infty} \step_{\run} = \infty$ and $\sum_{\run=\start}^{\infty} \step_{\run}^{2} < \infty$, we have $\lim_{\run\to\infty} \breg(\sol,\act_{\run})>0$ whenever $\act_{\start}\neq\sol$.
In words, $\act_{\run}$ always remains a positive distance away from $\sol$ if this is initially the case.
\end{proposition}

\begin{corollary}
In finite zero-sum games with a unique interior equilibrium, \eqref{eq:SPMD} cycles in perpetuity at positive Bregman distance from the game's equilibrium, even with perfect payoff observations.
\end{corollary}

\begin{proof}
Write $\payv_{1}(\state) = -\mat \state_{2}$ and $\payv_{2}(\state) = \state_{1}^{\top}\mat$ for the players' payoff vectors under the mixed strategy profile $\state = (\state_{1},\state_{2})$.
By construction, we have $\gvec(\state) = -(\payv_{1}(\state),\payv_{2}(\state))$.
Furthermore, since $\sol$ is an interior equilibrium of $\obj$, elementary game-theoretic considerations show that $\payv_{1}(\sol)$ and $\payv_{2}(\sol)$ are both proportional to the constant vector of ones.
We thus get
\begin{flalign}
\braket{\gvec(\state)}{\state-\sol}
	&= \braket{\payv_{1}(\state)}{\state_{1}-\sol_{1}}
	+ \braket{\payv_{2}(\state)}{\state_{2} - \sol_{2}}
	\notag\\
	&= -\state_{1}^{\top} \mat \state_{2} + (\sol_{1})^{\top} \mat \state_{2}
	+ \state_{1}^{\top} \mat \state_{2} - \state_{1}^{\top}\mat \sol_{2}
	\notag\\
	&= 0,
\end{flalign}
where, in the last line, we used the fact that $\sol$ is interior.

Now, as we show in the paper's supplement (\cref{prop:Bregman-new}), the evolution of the Bregman divergence under \eqref{eq:SPMD} satisfies the identity
\begin{flalign}
\label{eq:Bregman-lower}
\breg(\sol,\act_{\run+1})
	&= \breg(\sol,\act_{\run})
	+ \breg(\act_{\run},\act_{\run+1})
	+ \step_{\run} \braket{\gvec(\act_{\run})}{\act_{\run} - \sol}
	\notag\\
	&= \breg(\sol,\act_{\run}) + \breg(\act_{\run},\act_{\run+1})
	\notag\\
	&\geq \breg(\sol,\act_{\run}),
\end{flalign}
where, in the penultimate line, we used the fact that $\braket{\gvec(\state)}{\state-\sol} = 0$ for all $\state\in\feas$.
This shows that $\breg(\sol,\act_{\run})$ is nondecreasing.
%so, since $\breg(\sol,\act_{\start})>0$ by assumption, it follows that $\liminf_{\run\to\infty} \breg(\sol,\act_{\run}) > 0$.

Moreover, arguing as above and using \eqref{eq:Bregman-bound}, we also get
\begin{equation}
\breg(\sol,\act_{\run+1})
	\leq \breg(\sol,\act_{\run})
	+ \step_{\run}\braket{\gvec(\act_{\run})}{\act_{\run} - \sol}
	+ \frac{\step_{\run}^{2}}{2\strong} \dnorm{\gvec(\act_{\run})}^{2}
%	\notag\\
	\leq \breg(\sol,\act_{\run}) + \frac{\step_{\run}^{2}\gbound^{2}}{2\strong}
\end{equation}
with $\gbound = \max_{\state_{1}\in\feas_{1},\state_{2}\in\feas_{2}} \dnorm{(-\mat \state_{2},\state_{1}^{\top}\mat)}$.
Telescoping this last bound yields
\begin{equation}
\sup_{\run} \breg(\sol,\act_{\run})
	\leq \breg(\sol,\act_{\start}) + \sum_{\runalt=\start}^{\infty} \frac{\step_{\run}^{2}\gbound^{2}}{2\strong}
	< \infty,
\end{equation}
so $\breg(\sol,\act_{\run})$ is also bounded from above.
Therefore, with $\breg(\sol,\act_{\run})$ nondecreasing, bounded from above and $\breg(\sol,\act_{\start})>0$, it follows that $\lim_{\run\to\infty} \breg(\sol,\act_{\run}) > 0$, as claimed.
\end{proof}
